EACOF: A Framework for Providing Energy Transparency to enable Energy-Aware Software Development

Making energy consumption data accessible to software developers is an essential step towards energy efficient software engineering. The presence of various different, bespoke and incompatible, methods of instrumentation to obtain energy readings is currently limiting the widespread use of energy data in software development. This paper presents EACOF, a modular Energy-Aware Computing Framework that provides a layer of abstraction between sources of energy data and the applications that exploit them. EACOF replaces platform specific instrumentation through two APIs - one accepts input to the framework while the other provides access to application software. This allows developers to profile their code for energy consumption in an easy and portable manner using simple API calls. We outline the design of our framework and provide details of the API functionality. In a use case, where we investigate the impact of data bit width on the energy consumption of various sorting algorithms, we demonstrate that the data obtained using EACOF provides interesting, sometimes counter-intuitive, insights. All the code is available online under an open source license. http://github.com/eacof

==> results.tex <==
\section{Results}
\label{sec:results}

We have created \eacof, a framework which allows access to information about the energy consumption of software through the use of simple API calls.
This allows the development of code which may portably provide energy transparency to both the end user and developer.
In turn, it enables informed decisions to be made with respect to trade-offs regarding energy consumption.

\eacof is able to separate the two tasks of collecting and utilising dynamic energy consumption data through the use of \providers and \consumers.
This separation allows for a clear distinction of the two tasks, reducing the development overhead required for the successful completion of each task.
In addition, our design allows for functionality to improve over time without recompilation of all existing system components.

